Asynchronous Probabilistic Couplings in Higher-Order Separation Logic

Probabilistic couplings are the foundation for many probabilistic relational program logics and arise when relating random sampling statements across two programs. In relational program logics, this manifests as dedicated coupling rules that, e.g., say we may reason as if two sampling statements return the same value. However, this approach fundamentally requires aligning or "synchronizing" the sampling statements of the two programs which is not always possible. In this paper, we develop Clutch, a higher-order probabilistic relational separation logic that addresses this issue by supporting asynchronous probabilistic couplings. We use Clutch to develop a logical step-indexed logical relational to reason about contextual refinement and equivalence of higher-order programs written in a rich language with higher-order local state and impredicative polymorphism. Finally, we demonstrate the usefulness of our approach on a number of case studies. All the results that appear in the paper have been formalized in the Coq proof assistant using the Coquelicot library and the Iris separation logic framework.

==> sections/app-lazy-eager.tex <==
\section{Lazy/eager Coin}
In this section we give a more detailed proof of the lazy-eager coin example from \cref{sec:intro}.
We will go through the proof step by step but omit the use of \ruleref{rel-pure-l} and \ruleref{rel-pure-r} which should be interleaved with the application of most of the mentioned proof rules.

Recall the definitions
\begin{align*}
  \eagerprog \eqdef{}
  &\Let b = \Flip () in
  \Lam \_ . b \\
  \lazyprog \eqdef{}
  &\Let r = \Alloc(\None) in \\
  &\Lam \_ .
    \MatchML \deref r with
      \Some(b) => b
    | \None => {\begin{array}[t]{l}
      \Let b = \Flip \TT in \\
      r \gets \Some(b); \\
      b
    \end{array}}
    end {}
\end{align*}
%
The goal is to show $\ctxeq{}{\lazyprog}{\eagerprog}{\tunit \to \tbool}$ which we do by first showing $\ctxrefinesS{\lazyprog}{\eagerprog}{\tunit \to \tbool}$ and then $\ctxrefinesS{\eagerprog}{\lazyprog}{\tunit \to \tbool}$.

To show $\ctxrefinesS{\lazyprog}{\eagerprog}{\tunit \to \tbool}$, we first define an intermediate labeled version of $\lazyprog$:
%
\begin{align*}
  \lazyprog' \eqdef{}
  &\Let \lbl = \AllocTape in \\
  &\Let r = \Alloc(\None) in \\
  &\Lam \_ .
    \MatchML \deref r with
      \Some(b) => b
    | \None => {\begin{array}[t]{l}
      \Let b = \Flip(\lbl) in \\
      r \gets \Some(b); \\
      b
    \end{array}}
    end {}
\end{align*}
%
By transitivity of contextual refinement and \cref{thm:soundness} it is sufficient to show $\refines{}{\lazyprog}{\lazyprog'}{\tunit \to \tbool}$ and $\refines{}{\lazyprog'}{\eagerprog}{\tunit \to \tbool}$.

The first refinement $\refines{}{\lazyprog}{\lazyprog'}{\tunit \to \tbool}$ is mostly straightforward.
By applying \ruleref{rel-alloc-l} followed by \ruleref{rel-alloc-tape-r} and \ruleref{rel-alloc-r} we are left with the goal of proving that the two thunks are related, given $\spectape{\lbl}{1}{\nil}$, $\progheap{\loc}{\None}$ and $\specheap{\loc'}{\None}$ for some fresh label $\lbl$ and fresh locations on the heap $\loc$ and $\loc'$.
Using \ruleref{rel-na-inv-alloc} we allocate the invariant
%
\begin{align*}
  \spectape{\lbl}{1}{\nil} \sep (& (\progheap{\loc}{\None} \sep \specheap{\loc'}{\None}) \\
  &\lor{} (\Exists b. \progheap{\loc}{\Some(b)} \sep \specheap{\loc'}{\Some(b)}))
\end{align*}
%
with some name $\namesp$ that expresses how the $\lbl$ tape is always empty and that \emph{either} both $\loc$ and $\loc'$ contain $\None$ \emph{or} both contain $\Some(b)$ for some $b$.
We continue by \ruleref{rel-rec} after which we open the invariant and do a case distinction on the disjunction in the invariant.
If $\loc$ and $\loc'$ are empty, this is the first time we invoke the function.
We continue using \ruleref{rel-load-l} and \ruleref{rel-load-r}:
%
\begin{mathpar}
  \inferH{rel-load-l}
  {
    \progheap{\loc}{\val} \\
    \progheap{\loc}{\val} \wand \refines{\Delta}[\mask]{\fillctx\lctx[\val]}{\expr_2}{\type}
  }
  {\refines{\Delta}[\mask]{\fillctx\lctx[! \loc]}{\expr_2}{\type}} % spacing becomes a bit funny with \deref here
  %
  \and
  %
  \inferH{rel-load-r}
  {
    \specheap{\loc}{\val} \\
    \specheap{\loc}{\val} \wand \refines{\Delta}[\mask]{\expr_1}{\fillctx\lctx[\val]}{\type}
  }
  {\refines{\Delta}[\mask]{\expr_1}{\fillctx\lctx[! \loc]}{\type}} % spacing becomes a bit funny with \deref here
\end{mathpar}
after which we are left with the goal
%
\begin{align*}
  \refines{}[\top \setminus \namesp]
    {
  \begin{aligned}
    &\Let b = \Flip\TT in \\
    &r \gets \Some(b); b
  \end{aligned}
  }
  {
  \begin{aligned}
    &\Let b = \Flip(\lbl) in \\
    &r \gets \Some(b); b
  \end{aligned}
  }
  {\tunit \to \tbool}
\end{align*}
%
We continue using \ruleref{rel-rand-erase-r} to couple the two $\Flip$s, we follow by \ruleref{rel-store-l} and \ruleref{rel-store-r} to store the fresh bit on the heaps, we close the invariant (now showing the right disjunct as the locations have been updated) using \ruleref{rel-na-inv-close}, and we finish the case using \ruleref{rel-return} as the program returns the same Boolean $b$ on both sides.

If $\loc$ and $\loc'$ were \emph{not} empty, this is not the first time the function is invoked and we load the same Boolean on both sides using \ruleref{rel-load-l} and \ruleref{rel-load-r} and finish the proof using \ruleref{rel-na-inv-close} and \ruleref{rel-return}.

For the second refinement $\refines{}{\lazyprog'}{\eagerprog}{\tunit \to \tbool}$ we start by allocating the tape on the left using \ruleref{rel-alloc-tape-l} which gives us ownership of a fresh tape $\progtape{\lbl}{1}{\nil}$.
We now couple the $\lbl$ tape with the unlabeled $\Flip()$ on the right using \ruleref{rel-couple-tape-l}.
This gives us that for some $b$ then $\progtape{\lbl}{1}{b}$ and the $\Flip()$ on the right returned $b$ as well.
We continue by allocating the reference on the left using \ruleref{rel-alloc-l} which gives us some location $\loc$ and $\progheap{\loc}{\None}$.
Now, we allocate the invariant
\begin{align*}
  (\progtape{\lbl}{1}{b} \sep \progheap{\loc}{\None}) \lor \progheap{\loc}{\Some(b)}
\end{align*}
for some name $\namesp$ which expresses that \emph{either} the location $\loc$ is empty but $b$ is on the $\lbl$ tape, \emph{or} $b$ has been stored at $\loc$.
We are now left with proving that the two thunks are related under this invariant.
We continue using \ruleref{rel-rec} after which we open the invariant using \ruleref{rel-na-inv-open}, do a case distinction on the disjunction, and continue using \ruleref{rel-load-l}.
If the location $\loc$ is empty, we have to show
%
\begin{align*}
  \refines{}[\top \setminus \namesp]
    {
  \begin{aligned}
    &\Let b = \Flip(\lbl) in \\
    &r \gets \Some(b); b
  \end{aligned}
  }
  { b }
  {\tunit \to \tbool}
\end{align*}
But as we own $\progtape{\lbl}{1}{b}$ we continue using \ruleref{rel-rand-tape-l}, \ruleref{rel-store-l}, \ruleref{rel-na-inv-close} (now establishing the right disjunct as $\loc$ has been updated), and \ruleref{rel-return} as the return value $b$ is the same on both sides.
If the location $\loc$ was \emph{not} empty, we know $\progheap{\loc}{\Some(b)}$ which means \ruleref{rel-load-l} reads $b$ from $\loc$ and we finish the proof using \ruleref{rel-na-inv-close} (reestablishing the right disjunct) and \ruleref{rel-return}.

The proof of $\ctxrefinesS{\eagerprog}{\lazyprog}{\tunit \to \tbool}$ is analogous and we have shown the contextual equivalence of the programs $\eagerprog$ and $\lazyprog$.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../appendix"
%%% End:

